Compressed-Language Models for Understanding Compressed File Formats: a JPEG Exploration

This study investigates whether Compressed-Language Models (CLMs), i.e. language models operating on raw byte streams from Compressed File Formats~(CFFs), can understand files compressed by CFFs. We focus on the JPEG format as a representative CFF, given its commonality and its representativeness of key concepts in compression, such as entropy coding and run-length encoding. We test if CLMs understand the JPEG format by probing their capabilities to perform along three axes: recognition of inherent file properties, handling of files with anomalies, and generation of new files. Our findings demonstrate that CLMs can effectively perform these tasks. These results suggest that CLMs can understand the semantics of compressed data when directly operating on the byte streams of files produced by CFFs. The possibility to directly operate on raw compressed files offers the promise to leverage some of their remarkable characteristics, such as their ubiquity, compactness, multi-modality and segment-nature.

==> Sections/intro_bak.tex <==
% version as of may 14 20:00

\section{Introduction}
\textcolor{blue}{Paragraph 1: compressed file formats have nice properties + can be (collectively) considered as a language}\\
The digital world stores all of its information in files, where each individual file follows a fixed byte structure defined by its file format (\texttt{.doc}, \texttt{.wav}, \texttt{.avi}).
These formats allow for a standardized parsing process and predictive file writing into a byte stream, regardless of the storage device. 
To better handle storage and bandwidth limitations~\cite{????}, modern standards have defined Compressed File Formats (CFFs). 
This compressed disk representation cannot be directly read/parsed into the original file, a decoding process allows the translation from the compressed byte array into the original file structure/format. 
Given their versatility and general availability, CFFs have become fundamental in the digital world, where they are the de facto-standard for multi-media distribution and streaming \cite{}. 


We highlight three key characteristics of CFFs: 
i) \textbf{Ubiquity}: CFFs have become a standard, and can be found in public and private data collections everywhere.
(ii) \textbf{Compactness}: CFFs byte encoding typically reduces redundancy by exploiting statistical properties (\eg Huffman code in JPEG) or local repetitive patterns (\eg motion vectors in MPEG).
(iii) \textbf{Generality}: Although there are diverse compression methods, each individual encoding is versatile enough to map an arbitrary file (within a specific modality) to a one-dimensional byte array that uses a fixed alphabet (\textit{i.e.} Bits in the storage device).

The communication objective of CFFs, coupled with characteristics like syntax (the file structure of CFF is well defined), semantics (CFFs encode a media type), and finite lexicon (CFFS are represented with a finite set of unique bytes), suggests that CFFs are more than just a compact representation of multi-media files, and could be seen as an universal machine language that efficiently represents the corpora of digital media.

%suggests CFFs could be understood as the language that forms the corpora of digital media.
%CFFs are encoding designed for machines with the objective of efficiently storing and transmitting various kinds of information.

\textcolor{blue}{Paragraph 2: training on CFFs makes sense+offers advantages}\\

Recognizing language-like properties on CFFs implies that current language models (LMs) could be tuned to interpret the semantic information encoded on CFFs. % this ``CFF-ese''.
Moreover, 

a LM capable of working with compressed byte formats, should also be effective at manipulating these semantics without explicitly decoding the compressed byte stream. We will refer to such LM as the Compressed Language Model (CLM). A CLM would offer various advantages:
(1) \textbf{Compressed input}: compared to LMs operating on uncompressed formats (for example the pixel data of an image), a CLM would operate directly on a compact representation with minimal redundancy.
(2) \textbf{Raw input}: CLMs can leverage the vast corpora of compressed files, \textit{as stored}. Thus eliminating the codec-dependent pre-processing, and enabling semantic operations on partial inputs (\ie file segments, or streams).
(3) \textbf{Universality}: CLMs would allow a universal training pipeline: sequence-to-sequence models as a generic architecture, next-token prediction as the optimization objective, and CFFs as the standardized language for encoding and pre-processing information regardless of its nature (images, text, video, \etc).

%express essential information for reconstruction by reducing redundancy from statistical and local patterns, leaving only semantic redundancy,

\textcolor{blue}{paragraph 3: it's unclear if this language can be learned from files: the nature of CFFs may make learning challenging}\\
Despite the potential advantages of learning a generative language model on CFFs, it is still unknown if this language is learnable by directly training on the raw byte-streams that constitute CFFs. Various properties of CFFs make learning from them highly challenging. In particular, we note that these files have complex structures and are the result of layered compression strategies, where the original data undergoes a pipe-line of transformations to obtain the compressed representation. Moreover, their compressed nature implies that minimal alterations can drastically affect the global encoded information, and the reduced redundancy may hinder common self-supervised tasks such as mask-token prediction \cite{}. 

Further properties like lack of clear boundaries, complex entropy coding, high dimensionality, non-uniform distributions, and long-context-sensitive meanings all add to the difficulty of learning from CFFs.

\textcolor{blue}{paragraph 4: introduce the paper's focus and contributions}\\
In this paper, we study the feasibility of directly training generative language models for next-token prediction on raw byte streams from CFFs. 
To this end, we focus on the JPEG format as a case study for CFFs, given its commonality, how it exemplifies key concepts of CFFs, and the ease of evaluating generations via visual inspection.
Our contributions are threefold:
(1) \textbf{Framework}: we present a novel framework for generative pre-training of language models directly on CFF-encoded files, leveraging their compactness, raw format, and universal characteristics.
(2) \textbf{Evaluation}: 
(3) \textbf{Insights}: 



